Joint Depth and Normal Estimation from Real-world Time-of-flight Raw Data

We present a novel approach to joint depth and normal estimation for time-of-flight (ToF) sensors. Our model learns to predict the high-quality depth and normal maps jointly from ToF raw sensor data. To achieve this, we meticulously constructed the first large-scale dataset (named ToF-100) with paired raw ToF data and ground-truth high-resolution depth maps provided by an industrial depth camera. In addition, we also design a simple but effective framework for joint depth and normal estimation, applying a robust Chamfer loss via jittering to improve the performance of our model. Our experiments demonstrate that our proposed method can efficiently reconstruct high-resolution depth and normal maps and significantly outperforms state-of-the-art approaches. Our code and data will be available at \url{https://github.com/hkustVisionRr/JointlyDepthNormalEstimation}

==> vcl-shortcuts.tex <==
% This is roughly version 1.1 of vcl-shortcuts, circa Dec 2016.
% Put together by Vladlen Koltun

\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\usepackage[usenames, dvipsnames]{color}
\usepackage{nicefrac}

%Set up nice tables using the tabular package
%Make \toprule and \bottomrule thicker than \midrule
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%Set up the siunitx package, particularly for using the S column type in tables
\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries


%Known issue: the following shortcuts override \gg, \ll\, and \tt, which are existing LaTeX commands. Use \ggreater and \llesser, defined below, instead of \gg and \ll. Use \texttt{} instead of \tt.
%Also \ss is taken and in some environments cannot be overridden. Use \sss for a bold `s' instead.
\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

%\ggreater and \llesser replace \gg and \ll, which have been overridden
\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

%Checkmark and cross symbols for tables
\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}%

%Use @ instead of , in long numbers in math mode. For example, use $10@000$ rather than $10,000$.
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}

%Use \timess instead of \times in the main lines of equations, but not in superscripts or subscripts. Use the regular \times in superscripts or subscripts.
\newcommand\timess{\mathbin{\!\times\!}}

%Known issue: \nicebar is not nice in PNAS format, use \bar if submitting to PNAS.
\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

%Replace ``\yourname" and ``Name" with your name
\newcommand\qifeng[1]{\textcolor{blue}{Qifeng says: #1}}
\newcommand\vladlen[1]{\textcolor{blue}{Vladlen says: #1}}
\newcommand\xiaojuan[1]{\textcolor{blue}{Xiaojuan says: #1}}

%Paragraph heading with customizable vertical spacing. Modify the length inside \vspace to expand or contract the vertical offset preceding a new paragraph heading.
\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

%Orient text vertically. Useful for tables and figures.
\def\rot#1{\rotatebox{90}{#1}}

%I use the self-indulgent \LaTeX operator mostly to illustrate an issue and a useful trick. The issue is that LaTeX operators eat the space that follows them, so if they occur in the middle of a sentence they eliminate the space separating the following word. But you can't just insert a space will-nilly (e.g., \LaTeX\ or \LaTeX~) because if the operator is followed by a punctuation mark then there shouldn't be a space. One solution is to write \LaTeX{}, which does the right thing but is easy to forget. The alternative, demonstrated here, is to define an operator with a name that ends with the forward slash. This also does the right thing and looks sufficiently distinctive to be memorable.
\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}

%Miscellaneous \latex/ tips:
% To create an invisible character, use the \phantom command or its relatives: http://tex.stackexchange.com/questions/4519/how-do-i-create-an-invisible-character

